A Type System for Unstructured Locking that Guarantees Deadlock Freedom without Imposing a Lock Ordering

Deadlocks occur in concurrent programs as a consequence of cyclic resource acquisition between threads. In this paper we present a novel type system that guarantees deadlock freedom for a language with references, unstructured locking primitives, and locks which are implicitly associated with references. The proposed type system does not impose a strict lock acquisition order and thus increases programming language expressiveness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{K. Honda and A. Mycroft (Eds.): Programming Language\\
Approaches to Concurrency and communication-cEntric\\
Software 2010 (PLACES'10)\\
EPTCS 69, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.69.4}{10.4204/EPTCS.69.4}}

